A Unified Model and Dimension for Interactive Estimation

We study an abstract framework for interactive learning called interactive estimation in which the goal is to estimate a target from its "similarity'' to points queried by the learner. We introduce a combinatorial measure called dissimilarity dimension which largely captures learnability in our model. We present a simple, general, and broadly-applicable algorithm, for which we obtain both regret and PAC generalization bounds that are polynomial in the new dimension. We show that our framework subsumes and thereby unifies two classic learning models: statistical-query learning and structured bandits. We also delineate how the dissimilarity dimension is related to well-known parameters for both frameworks, in some cases yielding significantly improved analyses.

==> A6-DEC.tex <==


\subsection{Proof of Proposition \ref{prop:dec_sep}}

In this section we will prove the following Proposition.

\propositiondeccomparison*

We will exhibit a function class $\tilde{\mathcal{F}} \subset \F_{N, \epsilon}$ for which optimization over $\mathrm{conv}(\tilde{\mathcal{F}})$ is hard. Consider $ \{\xb_1, \cdots, \xb_N\}$ arbitrary distinct points in $\{ (\cos x, \sin x) : x \in \left(0, \pi \right) \}$ and $\vb = (0,1)$. Consider the subset $\tilde{\mathcal{F}} = \{ f_i^\vb , f_i^{-\vb}\}_{i=1}^N \subset \F_{0,N, \epsilon}$ of functions defined as
\begin{equation*}
f^\wb_i(\ab) = \begin{cases}
    \epsilon &\text{if }\ab = \xb_i\\
    -\epsilon &\text{if }\ab \in \{ \xb_j \}_{j=1}^N \backslash \{\xb_i\}\\
    0 &\text{if }\ab \in U_0\backslash S\\
    \langle \wb, \ab \rangle &\text{if }\ab \in \C \backslash U_0
    \end{cases}
\end{equation*}
with $\wb \in \{ \vb, -\vb\}$. Consider the function class $\F_{\mathrm{hard}} = \{ f_i \}_{i=1}^N$ with domain $\C$ consisting of the $N$ functions $f_i$ defined as,
\begin{equation*}
f_i(\ab) = \begin{cases}
    \epsilon &\text{if }\ab = \xb_i\\
    -\epsilon &\text{if }\ab \in \{ \xb_j \}_{j=1}^N \backslash \{\xb_i\}\\
    0 &\text{o.w.}
    \end{cases}
\end{equation*}
The function class $\F_{\mathrm{hard}}$ consists of `indicator functions' over each of the special points $ \{\xb_i\}_{i=1}^N$. Observe that $\F_{\mathrm{hard}} \subset  \mathrm{conv}(\tilde{F} )$. 





Notice that $f_i = \frac{1}{2} \left( f_i^\vb + f_i^{-\vb} \right) $ for all $i =1, \cdots, N$, proving that $\F_{\mathrm{hard}} \subset \mathrm{conv}(\F_{N, \epsilon})$. 


We turn our attention to the proof of Proposition~\ref{prop:dec_sep}. %

We will show that for any algorithm $\Alg$ there is $f^* \in \F_{\mathrm{hard}}$ such that $$\mathbb{E}_{{\Alg},f^*}\left[\mathrm{Regret}(T, \epsilon) \right]  \geq \Omega\left( \min(T, N) \epsilon \right).$$



We will imagine an experiment where the ground truth $f$ is chosen uniformly at random from $\mathcal{F}_{\mathrm{hard}}$ at the start of $\Alg$'s interaction with the environment. We use the notation $z_1, \cdots, z_T$ where $z_t=  (g_t, \ab_t) \in \mathrm{conv}(\tilde{F} ) \times \A$  to denote a (random) sample path of query tuples for algorithm $\Alg$ with observed responses $r_1, \cdots,r_T$ where $r_t = f(\ab_t) + \xi_t$. 


When $\Alg$ is interacting with an environment where $f = f_i \in \mathcal{F}_{\mathrm{hard}}$ and it produces a query point $\ab_t$ at time $t$, its instantaneous regret $\epsilon- \rho(z_t|(f_i, \xb_i )) = \max_{\ab \in \C} f_i(\ab) - f_i(\ab_t)$  is of order at least $\epsilon$ when $\ab_t \neq \xb_i$.


Define a stopping time $T_{\mathrm{opt}}$ as the first instant in $\Alg$'s sample path when $\ab_{T_{\mathrm{opt}}}$ is an optimal point of $f$ and satisfies $f(\ab_{T_{\mathrm{opt}}}) = \epsilon$. By definition, the regret of $\Alg$ over any sample path satisfies $\mathrm{Regret}(T, \epsilon) \geq \epsilon(T_{\mathrm{opt}} -1)$. We'll start by showing that, 
\begin{equation*}
    \mathbb{P}_{\Alg, f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}} )} \left( T_{\mathrm{opt}} \geq N/2\right) \geq (1-2/N)^{N/2} \geq 1/2e. 
\end{equation*}
Let $t \leq N/2$ and assume $z_1, \cdots, z_t$ is a sample path of query points for algorithm $\Alg$ such that $T_{\mathrm{opt}} > t$, that is the observed responses $r_1, \cdots,r_t$ satisfy $f(\ab_\ell) =-\epsilon$ for $\ab_\ell \in \{\xb_i\}_{i=1}^N$ and $f(\ab_\ell) =0$ for $\ab_\ell \not\in \{\xb_i\}_{i=1}^N$ for all $\ell \leq t$. Let $\tilde{\mathcal{F}}_t \subset \mathcal{F}_{\mathrm{hard}}$ be the set of functions $\tilde{f}$ such that $\tilde f(\ab_\ell) = f(\ab_\ell)$  for all $\tilde f \in \tilde{\mathcal{F}}_t$.  Since $t \leq N/2$ the set $\tilde{\mathcal{F}}_t$ satisfies $|\tilde{\mathcal{F}}_t| \geq N/2$ and therefore,
\begin{equation*}
    \mathbb{P}_{\Alg, f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}} )} \left(  T_{\mathrm{opt}} = t+1 \Bigg| T_{\mathrm{opt}} > t \right) \leq \frac{1}{|\tilde{\F}_t| } \leq \frac{2}{N}. 
\end{equation*}
This is because the conditional distribution over the set of functions that agree with the data up to time $t$ is uniform over $\tilde{\mathcal{F}}_t$. When $\ab_{t+1}$ is one of the points of $\{\xb_i\}_{i=1}^N$ that has not been selected by $\Alg$ during timesteps $1$ to $t$, the conditional probability of $T_{\mathrm{opt}} = t+1$ equals $\frac{1}{|\tilde{\mathcal{F}}_t|}$. For any other choice of $\ab_{t+1}$ the conditional probability of $T_{\mathrm{opt}} = t+1$ equals $0$. This implies that
\begin{equation*}
    \mathbb{P}_{\Alg, f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}} )} \left(  T_{\mathrm{opt}} > t+1 \Bigg|  T_{\mathrm{opt}} > t  \right) \geq 1-\frac{2}{N}. 
\end{equation*}
A simple inductive argument implies $$\mathbb{P}_{\Alg, f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}} )} \left(  T_{\mathrm{opt}} \geq \min( N/2, T) \right) \geq \left(1-\frac{2}{N}\right)^{\min(N/2, T)} \geq 1/2e.$$ 
Recall the regret of $\Alg$ over any sample path satisfies $\mathrm{Regret}(T, \epsilon) \geq \epsilon(T_{\mathrm{opt}} -1)$. Therefore,
\begin{align*}
    \mathbb{E}_{f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}})}&\left[\mathbb{E}_{{\Alg},f} \left[ \mathrm{Regret}(T, \epsilon)\right] \right] \\
    &\geq \mathbb{E}_{f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}})}\left[\epsilon \cdot ( T_\mathrm{opt} -1)\right] \\
    &\geq   \mathbb{P}_{\Alg, f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}} )}\left( T_{\mathrm{opt}} \geq \min(N/2, T)\right)  \cdot \epsilon \cdot  (\min(N/2, T) -1) \\
    &\geq \frac{ (\min(N/2, T) -1) \epsilon }{2e}\\
    &\geq \Omega(\min(T, N)\epsilon).
\end{align*}

This implies that $\Alg$'s regret over uniform random choices $f \sim \mathrm{Uniform}(\mathcal{F}_{\mathrm{hard}})$ is at least $\Omega( \min(T, N) \epsilon  )$. Finally, this implies there exists a function $f^* \in \mathcal{F}_{\mathrm{hard}} \subset \mathrm{conv}(\mathcal{F}_{N, \epsilon})$ such that $\mathbb{E}_{{\Alg},f^*}[ \mathrm{Regret}(T, \epsilon) ] \geq \Omega\left( \min(T, N) \epsilon \right)$ where $\mathbb{E}_{{\Alg},f^*}[\cdot]$ corresponds to the expectation of using algorithm $\Alg$ with action space $\C$ when the true function equals $f^*$. 

Let $\tilde{Z} = \tilde \F \times \A$. In contrast Theorem~\ref{thm:regret_optimism} and Proposition~\ref{prop::separation_eluder_dissimilarity} imply that Algorithm~\ref{alg:MAIN1} ($\Alg_1$) will satisfy a regret bound of $\mathrm{Regret}(T,\alpha)= O(\d^{3/2}_{\score}(\tilde{\Z}, 1, \epsilon) ) = O(\sqrt{C_{T,\delta} \ T})$ with $C_{T,\delta} = O( \log(TN/\delta))$ (since $\tilde F$ is of finite of size $N$) with probability $1-\delta$. Setting $\delta = 1/T$ implies that for all $f \in \tilde{F}$, $\mathbb{E}_{\Alg_1, f}[ \mathrm{Regret}(T, 1)] \leq O(\sqrt{\log(TN) \ T})$ and the result follows. 
 




